A Convex Parameterization of Controllers Constrained to use only Relative Measurements

The optimal controller design problem for systems equipped with sensors that measure only relative, rather than absolute, quantities is considered. This relative measurement structure is formulated as a design constraint; it is demonstrated that the resulting constrained controller design problem can be written as a convex program. Certain additional network structural constraints can be incorporated into this formulation, making it especially useful in distributed or networked settings. An illustrative example highlights the advantage of the proposed methodology over the standard formulation of the output feedback controller design problem. A numerical example is provided.

==> bibliography.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% https://bibdesk.sourceforge.io/

%% Created for Emily Jensen at 2023-04-11 11:46:17 -0700 


%% Saved with string encoding Unicode (UTF-8) 


@article{zelazo2010graph,
  title={Graph-theoretic analysis and synthesis of relative sensing networks},
  author={Zelazo, Daniel and Mesbahi, Mehran},
  journal={IEEE Transactions on Automatic Control},
  volume={56},
  number={5},
  pages={971--982},
  year={2010},
  publisher={IEEE}
}


@article{rotkowitz2005characterization,
  title={A characterization of convex problems in decentralized control},
  author={Rotkowitz, Michael and Lall, Sanjay},
  journal={IEEE transactions on Automatic Control},
  volume={50},
  number={12},
  pages={1984--1996},
  year={2005},
  publisher={IEEE}
}


@inproceedings{jensen2020gap,
  title={On the gap between system level synthesis and structured controller design: the case of relative feedback},
  author={Jensen, Emily and Bamieh, Bassam},
  booktitle={2020 American Control Conference (ACC)},
  pages={4594--4599},
  year={2020},
  organization={IEEE}
}

@article{jovanovic2005ill,
  title={On the ill-posedness of certain vehicular platoon control problems},
  author={Jovanovic, Mihailo R and Bamieh, Bassam},
  journal={IEEE Transactions on Automatic Control},
  volume={50},
  number={9},
  pages={1307--1321},
  year={2005},
  publisher={IEEE}
}


@article{psiaki1999autonomous,
  title={Autonomous orbit determination for two spacecraft from relative position measurements},
  author={Psiaki, Mark L},
  journal={Journal of Guidance, Control, and Dynamics},
  volume={22},
  number={2},
  pages={305--312},
  year={1999}
}


@article{sarlette2014control,
  title={Control limitations from distributed sensing: Theory and extremely large telescope application},
  author={Sarlette, Alain and Sepulchre, Rodolphe J},
  journal={Automatica},
  volume={50},
  number={2},
  pages={421--430},
  year={2014},
  publisher={Elsevier}
}


@book{mesbahi2010graph,
  title={Graph theoretic methods in multiagent networks},
  author={Mesbahi, Mehran and Egerstedt, Magnus},
  year={2010},
  publisher={Princeton University Press}
}

@book{francis1987course,
  title={A course in H$\infty$ control theory},
  author={Francis, Bruce A},
  year={1987},
  publisher={Springer}
}

@article{bamieh2002distributed,
  title={Distributed control of spatially invariant systems},
  author={Bamieh, Bassam and Paganini, Fernando and Dahleh, Munther A},
  journal={IEEE Transactions on automatic control},
  volume={47},
  number={7},
  pages={1091--1107},
  year={2002},
  publisher={IEEE}
}

@artice{vamsi2016network,
  author={Mohan Vamsi, Andalam Satya and Elia, Nicola},
  journal={IEEE Transactions on Automatic Control}, 
  title={Optimal Distributed Controllers Realizable Over Arbitrary Networks}, 
  year={2016},
  volume={61},
  number={1},
  pages={129-144},
  doi={10.1109/TAC.2015.2434051}
}


@book{dullerud2013course,
  title={A course in robust control theory: a convex approach},
  author={Dullerud, Geir E and Paganini, Fernando},
  volume={36},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@article{bamieh2005convex,
  title={A convex characterization of distributed control problems in spatially invariant systems with communication constraints},
  author={Bamieh, Bassam and Voulgaris, Petros G},
  journal={Systems \& control letters},
  volume={54},
  number={6},
  pages={575--583},
  year={2005},
  publisher={Elsevier}
}


@INPROCEEDINGS{karimian2020consensus,
  author={Karimian, Arman and Tron, Roberto},
  booktitle={2020 American Control Conference (ACC)}, 
  title={Bearing-Only Consensus and Formation Control under Directed Topologies}, 
  year={2020},
  volume={},
  number={},
  pages={3503-3510},
  doi={10.23919/ACC45564.2020.9147417}
}

@ARTICLE{tang2018harmonic,
  author={Song, Qiang and Liu, Fang and Cao, Jinde and Vasilakos, Athanasios V. and Tang, Yang},
  journal={IEEE Transactions on Control of Network Systems}, 
  title={Leader-Following Synchronization of Coupled Homogeneous and Heterogeneous Harmonic Oscillators Based on Relative Position Measurements}, 
  year={2019},
  volume={6},
  number={1},
  pages={13-23},
  doi={10.1109/TCNS.2018.2791204}
}

@article{trinh2018bearing,
  title={Bearing-based formation control of a group of agents with leader-first follower structure},
  author={Trinh, Minh Hoang and Zhao, Shiyu and Sun, Zhiyong and Zelazo, Daniel and Anderson, Brian DO and Ahn, Hyo-Sung},
  journal={IEEE Transactions on Automatic Control},
  volume={64},
  number={2},
  pages={598--613},
  year={2018},
  publisher={IEEE}
}

@book{bullo2020lectures,
  title={Lectures on network systems},
  author={Bullo, Francesco},
  volume={1},
  number={3},
  year={2020},
  publisher={Kindle Direct Publishing Seattle, DC, USA}
}
@article{tegling2015price,
  title={The price of synchrony: Evaluating the resistive losses in synchronizing power networks},
  author={Tegling, Emma and Bamieh, Bassam and Gayme, Dennice F},
  journal={IEEE Transactions on Control of Network Systems},
  volume={2},
  number={3},
  pages={254--266},
  year={2015},
  publisher={IEEE}
}

@inproceedings{oral2019disorder,
  title={Disorder in large-scale networks with uni-directional feedback},
  author={Oral, H Giray and Gayme, Dennice F},
  booktitle={2019 American Control Conference (ACC)},
  pages={3394--3401},
  year={2019},
  organization={IEEE}
}

@article{tegling2017coherence,
  title={On the coherence of large-scale networks with distributed PI and PD control},
  author={Tegling, Emma and Sandberg, Henrik},
  journal={IEEE control systems letters},
  volume={1},
  number={1},
  pages={170--175},
  year={2017},
  publisher={IEEE}
}

@article{smith2005control,
  title={Control of deep-space formation-flying spacecraft; relative sensing and switched information},
  author={Smith, Roy S and Hadaegh, Fred Y},
  journal={Journal of Guidance, Control, and Dynamics},
  volume={28},
  number={1},
  pages={106--114},
  year={2005}
}

@article{wang2019system,
  title={A system-level approach to controller synthesis},
  author={Wang, Yuh-Shyang and Matni, Nikolai and Doyle, John C},
  journal={IEEE Transactions on Automatic Control},
  volume={64},
  number={10},
  pages={4079--4093},
  year={2019},
  publisher={IEEE}
}

@article{youla1976modern,
  title={Modern Wiener-Hopf design of optimal controllers--Part II: The multivariable case},
  author={Youla, Dante and Jabr, Hamid and Bongiorno, Jr},
  journal={IEEE Transactions on Automatic Control},
  volume={21},
  number={3},
  pages={319--338},
  year={1976},
  publisher={IEEE}
}

@article{park2023skin,
  title={Skin-integrated systems for power efficient, programmable thermal sensations across large body areas},
  author={Park, Minsu and Yoo, Jae-Young and Yang, Tianyu and Jung, Yei Hwan and V{\'a}zquez-Guardado, Abraham and Li, Shupeng and Kim, Jae-Hwan and Shin, Jaeho and Maeng, Woo-Youl and Lee, Geumbee and others},
  journal={Proceedings of the National Academy of Sciences},
  volume={120},
  number={6},
  pages={e2217828120},
  year={2023},
  publisher={National Acad Sciences}
}

@article{wang2018toward,
  title={Toward perceptive soft robots: Progress and challenges},
  author={Wang, Hongbo and Totaro, Massimo and Beccai, Lucia},
  journal={Advanced Science},
  volume={5},
  number={9},
  pages={1800541},
  year={2018},
  publisher={Wiley Online Library}
}

@article{dullerud2004distributed,
  title={Distributed control of heterogeneous systems},
  author={Dullerud, Geir E and D'Andrea, Raffaello},
  journal={IEEE Transactions on Automatic Control},
  volume={49},
  number={12},
  pages={2113--2128},
  year={2004},
  publisher={IEEE}
}

@article{nayyar2013decentralized,
  title={Decentralized stochastic control with partial history sharing: A common information approach},
  author={Nayyar, Ashutosh and Mahajan, Aditya and Teneketzis, Demosthenis},
  journal={IEEE Transactions on Automatic Control},
  volume={58},
  number={7},
  pages={1644--1658},
  year={2013},
  publisher={IEEE}
}

@inproceedings{mahajan2012information,
  title={Information structures in optimal decentralized control},
  author={Mahajan, Aditya and Martins, Nuno C and Rotkowitz, Michael C and Y{\"u}ksel, Serdar},
  booktitle={2012 IEEE 51st IEEE Conference on Decision and Control (CDC)},
  pages={1291--1306},
  year={2012},
  organization={IEEE}
}

@inproceedings{ahsun2006dynamics,
  title={Dynamics and control of electromagnetic satellite formations},
  author={Ahsun, Umair and Miller, David W},
  booktitle={2006 American Control Conference},
  pages={6--pp},
  year={2006},
  organization={IEEE}
}

@article{abbasi2022decentralized,
  title={Decentralized Electromagnetic Formation Flight Using Alternating Magnetic Field Forces},
  author={Abbasi, Zahra and Hoagg, Jesse B and Seigler, T Michael},
  journal={IEEE Transactions on Control Systems Technology},
  volume={30},
  number={6},
  pages={2480--2489},
  year={2022},
  publisher={IEEE}
}

@inproceedings{correll2014soft,
  title={Soft autonomous materials—using active elasticity and embedded distributed computation},
  author={Correll, Nikolaus and {\"O}nal, {\c{C}}a{\u{g}}da{\c{s}} D and Liang, Haiyi and Schoenfeld, Erik and Rus, Daniela},
  booktitle={Experimental Robotics: The 12th International Symposium on Experimental Robotics},
  pages={227--240},
  year={2014},
  organization={Springer}
}

@article{kim2013soft,
  title={Soft robotics: a bioinspired evolution in robotics},
  author={Kim, Sangbae and Laschi, Cecilia and Trimmer, Barry},
  journal={Trends in biotechnology},
  volume={31},
  number={5},
  pages={287--294},
  year={2013},
  publisher={Elsevier}
}

